Scylla IV: Intrinsic Stellar Properties and Line-of-Sight Dust Extinction Measurements Towards 1.5 Million Stars in the SMC and LMC

By analyzing the spectral energy distributions (SEDs) of resolved stars in nearby galaxies, we can constrain their stellar properties and line-of-sight dust extinction. From the Scylla survey, we obtain ultraviolet to near-infrared photometry from Wide Field Camera 3 onboard the {\it Hubble Space Telescope} for more than 1.5 million stars in the SMC and LMC. We use the Bayesian Extinction and Stellar Tool (BEAST) to analyze the multi-band SEDs of these sources and characterize their initial masses, ages, metallicities, distances, and line-of-sight extinction properties (e.g.~$A_V$, $R_V$). We apply quality cuts and perform validation simulations to construct a catalog of over 550,000 stars with high-reliability SED fits, which we use to analyze the stellar content and extinction properties of the SMC and LMC. We detect stars with masses as low as 0.6 $M_{\odot}$. BEAST stellar age distributions show a jump in observed stars around 6 Gyrs ago, which agrees with star-formation histories. Extinctions ($A_V$) in both galaxies follow a log-normal distribution. We compare $A_V$ with ancillary gas and dust tracers like $HI$, $H_\alpha$, and far infrared (FIR) dust emission and find positive correlations on a field-by-field basis. We convert observed $A_V$ to predicted dust surface densities using the Draine et. al. (2014) model and find $A_V$-based dust surface densities are a factor of $\sim$2.5 lower than observed FIR-based dust surface densities, a correction factor similar to other studies.

==> description_of_beast_columns.tex <==
Column Descriptions for the Catalog
A listing of the columns in the catalog is provided below. The team has added brief descriptions of the general columns here. For further information regarding the BEAST parameters, users should consult the official BEAST documentation (https://beast-docs.readthedocs.io/en/latest).

General Parameters
- Name: IAU suggested naming scheme used (example: PHAT J113759.63+421022.03)
- RA: right ascension from photometry catalog
- DEC: declination from photometry catalog
- k30: KDE stellar density of massive stars using k=30 pc
- k100: KDE stellar density of massive stars using k=100 pc
- k300: KDE stellar density of massive stars using k=300 pc
- rad_dist: radial distance from the center of M31 in units of kpc
- nearest_d: distance to other nearest massive star in catalog in units of pc
- D15_Av: median of log-normal A(V) fit derived from PHAT RGB stars; corresponding total column density extinction from Dalcanton+15
- D15_sigma: sigma of log-normal A(V) fit derived from PHAT RGB stars; corresponding total column density extinction from Dalcanton+15
- K21_HI: corresponding HI 21-cm integrated intensity emission from Koch+21 in units of K km/(s)
- S21_CO: corresponding predicted CO(J=3-2) line flux from the HASHTAG survey (Smith+21) in units of K km/(s)

Fluxes
- HST_WFC3_F275W: fluxes in units of ergs/(cm^2 s A)
- HST_WFC3_F336W: fluxes in units of ergs/(cm^2 s A)
- HST_ACS_WFC_F475W: fluxes in units of ergs/(cm^2 s A)
- HST_ACS_WFC_F814W: fluxes in units of ergs/(cm^2 s A)
- HST_WFC3_F110W: fluxes in units of ergs/(cm^2 s A)
- HST_WFC3_F160W: fluxes in units of ergs/(cm^2 s A)

Vega Magnitudes
- F275W_VEGA: apparent magnitude derived from fluxes
- F336W_VEGA: apparent magnitude derived from fluxes
- F475W_VEGA: apparent magnitude derived from fluxes
- F814W_VEGA: apparent magnitude derived from fluxes
- F110W_VEGA: apparent magnitude derived from fluxes
- F160W_VEGA: apparent magnitude derived from fluxes

BEAST Fitted and derived parameter suffixes
- X_Exp: expectation value (average weighted by 1D PDF) 
- X_p50: 50th percentile from 1D PDF
- X_p16: 16th percentile from 1D PDF (p50-p16 is proxy for -1 sigma)
- X_p84: 84th percentile from 1D PDF (p84-p50 is proxy for +1 sigma)
- X_Best: single best BEAST model fit value from chi2min

BEAST Dust Parameters
- Av: A(V) visual extinction in magnitudes
- Rv: R(V) = A(V)/E(B-V) = ratio of total to selective extinction
- f_A: fraction in extinction curve from A component (MW)
- Rv_A: R(V)_A = R(V) of A component of BEAST R(V)-f_A model of extinction curves

BEAST Stellar Parameters
- M_ini: initial stellar mass (in solar masses)
- logA: log10 of the stellar age (in years)
- Z: stellar metallicity
- M_act: current stellar mass (in solar masses)
- logL: log10 of the stellar luminosity (in solar luminosities)
- logT: log10 of the stellar effective temperature (in Kelvin)
- logg: log10 of the stellar surface gravity (cm s^-2)
- mbol: bolometric magnitude
- radius: stellar radius (in solar radii)

BEAST Goodness-of-fit Metrics
- Pmax: maximum probability of nD PDF
- Pmax_indx: index in BEAST model grid corresponding to Pmax
- specgrid_indx: index in spectroscopic grid corresponding to Pmax
- chi2min: minimum value of chisqr
- chi2min_indx: index in BEAST model grid corresponding to chi2min

BEAST Predicted Fluxes
- logHST_WFC3_FXXXW_nd: log10 of the unextinguished (no dust) predicted flux for filters from WFC3
- logHST_WFC3_FXXXW_wd: log10 of the extinguished (with dust) predicted flux for filters from WFC3
- logHST_ACS_WFC_FXXXW_nd: log10 of the unextinguished (no dust) predicted flux for filters from ACS WFC
- logHST_ACS_WFC_FXXXW_wd: log10 of the extinguished (with dust) predicted flux for filters from ACS WFC
- logGALEX_FUV_nd: log10 of the unextinguished (no dust) GALEX FUV predicted flux
- logGALEX_FUV_wd: log10 of the extinguished (with dust) GALEX FUV predicted flux
- logGALEX_NUV_nd: log10 of the unextinguished (no dust) GALEX NUV predicted flux
- logGALEX_NUV_wd: log10 of the extinguished (with dust) GALEX NUV predicted flux
- logF_UV_6_13e_nd: log10 of the unextinguished (no dust) predicted flux between 6 and 13 eV
- logF_UV_6_13e_wd: log10 of the extinguished (with dust) predicted flux between 6 and 13 eV
